High order entropy preserving ADER scheme

In this paper, we develop a fully discrete entropy preserving ADER-Discontinuous Galerkin (ADER-DG) method. To obtain this desired result, we equip the space part of the method with entropy correction terms that balance the entropy production in space, inspired by the work of Abgrall. Whereas for the time-discretization we apply the relaxation approach introduced by Ketcheson that allows to modify the timestep to preserve the entropy to machine precision. Up to our knowledge, it is the first time that a provable fully discrete entropy preserving ADER-DG scheme is constructed. We verify our theoretical results with various numerical simulations.

==> ADER_DG.tex <==

\subsection{Notation}

This section introduces the basic notation used throughout the paper. 
As mentioned before, we follow the recent interpretation of ADER-DG as an explicit space-time FE discretization. 
We divide the spatial domain $\Omega$ into cells $\Omega_i$ (in our case triangles).
The numerical solution is represented by piecewise polynomials of degree $N \geq 0$ at time level $t^n$ and it is defined by 
\begin{equation}
\mathbf{u}_h^n(\x,t^n) = \sum \limits_{\ell=0}^{\mathcal{N}-1} \phi_\ell(\x) \, \hat{\mathbf{u}}^{n}_{\ell,i} 
, \qquad \x \in \Omega_i,
\label{eqn.uh}
\end{equation}
where $ \phi_\ell(\x) $ is a modal spatial basis and 
$\mathcal{N}$ denotes the total number of expansion coefficients  $\hat{\mathbf{u}}^{n}_{l}$.
%with respect to the degrees of freedom inside one cell. 
The basis function $\phi_\ell(\x) $ is defined through a Taylor series of degree $N$ in the cell $\Omega_i$. Let $\xbi$ be the barycenter of $\Omega_i$ and $h_i$ be the radius of the circumscribed circle around the triangle $\Omega_i$. The basis in $\Omega_i$ is given by  
\begin{equation} 
\label{eq.Dubiner_phi_spatial}
\phi_\ell(\x) = \frac{(x - x_{\mathbf{b}_i})^{p_\ell}}{p_\ell! \, h_i^{p_\ell}} \, \frac{(y - y_{\mathbf{b}_i})^{q_\ell}}{q_\ell! \, h_i^{q_\ell}}, \quad 
\ell = 0, \dots, \mathcal{N}-1, \quad  0 \leq p_\ell + q_\ell \leq N \quad \text{with} \quad \mathcal{N}= \frac{1}{d!} \prod \limits_{m=1}^{d} (N+m).
\end{equation} 
\begin{remark}[Extension to the general $P_NP_M$ framework]
If we choose $N=0$, we obtain as usual a first order FV method. Instead of increasing now the order of accuracy in one cell by setting $N>0$, one can,  for instance, apply a higher-order FV reconstruction up to order $M+1$. 
Therefore, our method is included in the more general class of $P_NP_M$ schemes proposed 
in~\cite{Dumbser20088209} and further developed in \cite{gaburro2021posteriori,gaburro2020high} which unifies higher-order FV and DG schemes into a common framework. Since the application of the entropy correction term inside a  FV scheme is more problematic as described in \cite{abgrall2022reinterpretation}, we restrict ourself in this paper on the ADER-DG approach only. Extensions to general $P_NP_M$ are planned for future  work. 
\end{remark}

Differently from classical Runge-Kutta discontinuous Galerkin method, the ADER-DG approach is not build on a method of line (MOL) ansatz but on a local predictor-corrector approach. The advantage of the predictor-corrector procedure is that the information exchange between the elements is done only once at each time step, only during the corrector step. This results in advantages in runtime and efficiency of the scheme \cite{balsara2013efficient}.
Therefore, we also define a space-time basis which  locally approximates our predictor $\q_h$ inside the element $C_i^n=\Omega_i \times [t^n,t^{n+1}]$. It is given by 
\begin{equation} 
\q_h^n(\x, t) = \sum_{\ell=0}^{\mathcal{Q}-1} \theta_\ell (\x, t) \hat{\q}_\ell^n, \quad (\x,t) \in C_i^n,  
\label{eqn.qh}
\end{equation} 
where  
\begin{equation}
\begin{aligned}
\label{eq.Dubiner_phi}
& \theta_\ell(x,y,t)|_{C_i^n} = \frac{(x -  x_{\mathbf{b}_i})^{p_\ell}}{{p_\ell}! \, h_i^{p_\ell}} \, \frac{(y -  y_{\mathbf{b}_i})^{q_\ell}}{{q_\ell}! \, h_i^{q_\ell}}
\, \frac{(t - t^n)^{r_\ell}}{{r_\ell}! \, h_i^{r_\ell}}, \\
& \ell = 0, \dots, \mathcal{Q}, 
\quad 0 \leq p_\ell + q_\ell + r_\ell \leq N \quad \text{with} \quad \mathcal{Q}= \frac{1}{(d+1)!} \prod \limits_{m=1}^{d+1} (N+m)
\end{aligned}
\end{equation} 
is our \textit{modal space--time} basis for the polynomials of degree $N$. Here, $\mathcal{Q}$ is the number of degrees of freedom in one space-time cell $C_i$.

\subsection{ADER-DG method}\label{subsec.ADER-DG}

ADER-DG schemes consist in two steps for the update of one timestep: the local predictor and the corrector, which we describe now separately.
\subsubsection{Local Predictor Step}
The method starts by calculating a high-order local predictor solution of the underlying PDE \eqref{eq.generalform}  using a classical Galerkin approach inside each element $C_i$. We obtain  
\begin{equation}
 \int_{t^n}^{t^{n+1}} \!\! \int_{\Omega_i^{\circ} } \theta_k \, \partial_t \q_h \,\diff \x \, \diff t 
+ \int_{t^n}^{t^{n+1}} \!\! \int_{\Omega_i^{\circ} } \theta_k \,\div \F(\q_h) \, \diff \x \,\diff t
= \mathbf{0}
\label{eq.predictorEq}
\end{equation}
with  $\Omega_i^{\circ} = \Omega_i \backslash \partial \Omega_i$ being the interior of the spatial cell.\\
Applying integration by parts in time yields finally 
\begin{equation}
\begin{aligned}
& \int_{\Omega_i^{\circ}}  \theta_k(\x,t^{n+1}) \q_h(\x,t^{n+1}) \, \diff \x -
\int_{\Omega_i^{\circ}} \theta_k(\x,t^{n}) \u_h(\x,t^{n}) \, \diff \x - \\
&\int_{t^n}^{t^{n+1}} \!\!\!  \int_{\Omega_i^{\circ} } \!\!\! \partial_t \theta_k(\x,t) \q_h(\x,t)  \diff \x \,\diff t + 
\int_{t^n}^{t^{n+1}} \!\!\!  \int_{\Omega_i^{\circ} } \!\!\! \theta_k(\x,t) \div\F(\q_h(\x,t))  \diff \x \,\diff t
= \mathbf{0},
\label{eq:DOFpredictor}
\end{aligned}
\end{equation}
in which now $\u_h(\x,t^{n})$ is given. Equation \eqref{eq:DOFpredictor} involves only the local polynomial $\q_h^n$ within a single  space-time element.
The space-time  predictors \eqref{eq:DOFpredictor} can be thus solved independently in each element. In practice,
we approximate their solution 
%which contains only local information and it is solved 
by a simple fixed-point iteration procedure (discrete Picard iterations) as follows
\begin{equation}
	\begin{aligned}
		& \int_{\Omega_i^{\circ}}  \theta_k(\x,t^{n+1}) \q_h^{(k+1)}(\x,t^{n+1}) \, \diff \x -
		\int_{t^n}^{t^{n+1}} \!\!\!  \int_{\Omega_i^{\circ} } \!\!\! \partial_t \theta_k(\x,t) \q_h^{(k+1)}(\x,t)  \diff \x \,\diff t =\\
		&\int_{\Omega_i^{\circ}} \theta_k(\x,t^{n}) \u_h(\x,t^{n}) \, \diff \x + 
		\int_{t^n}^{t^{n+1}} \!\!\!  \int_{\Omega_i^{\circ} } \!\!\! \theta_k(\x,t) \div\F(\q_h^{(k)}(\x,t))  \diff \x \,\diff t.
		\label{eq:DOFpredictor1}
	\end{aligned}
\end{equation} 
For further details one can refer to \cite{gaburro2020high,gaburro2021unified} where the same notation has been used.

\subsubsection{Corrector Step}

Once the  local space-time prediction of the  solution  $\q_h^n(\x, t) $ has been computed, we can write a one step  update in time as follows. We
 start by multiplying \eqref{eq.generalform} with  a spatial-only test function  $\phi_k$ (cf. equation \eqref{eq.Dubiner_phi_spatial}), and integrate in space and time: 
\begin{equation}
\int_{t^n}^{t^{n+1}} \int_{\Omega_i} \phi_k \left(\partial_t \u  + \div \F(\u) 
\right)   \diff \x \,\diff t
= \mathbf{0}.
\label{eqn.pde.weak}
\end{equation}
Inserting now \eqref{eqn.uh} in the time evolution variable and our local information \eqref{eq:DOFpredictor} in the flux, we can apply the divergence theorem in \eqref{eqn.pde.weak}, and we get our final update step of
the ADER-DG method:
\begin{equation}
\begin{aligned}
& \left( \, \int_{\Omega_i} \phi_k \phi_l \, d\x\right)
\left( \hat{\u}_\ell^{n+1} - \hat{\u}_\ell^{n} \, \right) 
+ \int_{t^n}^{t^{n+1}} \!\! \int_{\partial \Omega_i} \!\! \phi_k \mathcal{F}\left(\q_h^-, \q_h^+ \right) \cdot \mathbf{n} \, \diff S \, dt \ - 
 \int_{t^n}^{t^{n+1}} \!\! \int_{\Omega_i } \nabla \phi_k \cdot \F(\q_h)  \diff \x \,\diff t 
\, =\,  \mathbf{0},
\label{eq:ADER-DG}
\end{aligned}
\end{equation}
where $\mathcal{F}$ is the numerical flux, and $\mathbf{n}$ the external normal vector at the boundaries of the cell. Since we have the local predictor information $\q_h$, we can apply high-order quadrature rules for the approximation of time-integrals in \eqref{eq:ADER-DG} and we finally obtain our update for the solution at $t^{n+1}$. We remark that the information exchange in-between the elements plays a role only in the corrector step. 
As mentioned before, the presented interpretation of ADER-DG is an explicit space-time FE method. 




==> Entropy_ADER_DG.tex <==
As described in the previous section, the ADER-DG approach consists of two steps:
a set of  local predictors, and a fully explicit global corrector. The corrector step enforces
conservation, and thus consistency with weak solutions of \eqref{eq.generalform}.
%the corrector step
% Subsection \ref{subsec.ADER-DG}, the ADER-DG approach contains 
%two steps. 
%In the predictor step \eqref{eq:DOFpredictor1} the local approximations are calculated via a fixed-point iteration, while, in the final corrector step \eqref{eq:ADER-DG}, this local information is used to update solution at the next time step via communication between elements, always ensuring conservation. 
However, the entropy (in)equality \eqref{eq.generalform_entropy_conservation} (or \eqref{eq.generalform_entropy_inequality}) might not be guaranteed. 
Due to the  inherent space-time nature of the method, to enforce this additional constraint 
we need to have simultaneous control  of the  entropy production in space and in time.  
%method To obtain a \MR{fully discrete} entropy preserving scheme, we have to take care of the entropy production contributions in time and space inside the ADER-DG method.
%Mimicking the entropy property in the continuous setting, 
To this end we extend  two %we apply 
%two known 
techniques  previously proposed in literature: %oguarantee the preservation (dissipation) of the 
%entropy in space and in time: %, respectively:
\begin{enumerate}
\item for the balance of the spatial discretization in our ADER-DG method \eqref{eq:ADER-DG}, we apply entropy correction terms first proposed by Abgrall in \cite{abgrall2018general},
\item for handling the time-integration we deal with the relaxation approach described in \cite{ketcheson2019relaxationRK, ranocha2020relaxationMultistep}.
\end{enumerate}
In the following section %part, 
we explain how these techniques can be adapted to \eqref{eq:ADER-DG}. %our method \eqref{eq:ADER-DG}.

\subsection{Entropy correction in space}

The approach proposed by Abgrall in \cite{abgrall2018general} is based on the following idea. We introduce
a simple entropy correction term to the underlying discretization which is lead by a parameter which varies in every cell. 
The parameter is chosen in order to locally balance the entropy production at every degree of freedom and, simultaneously, not to violate the conservation property of the scheme. 
It can be interpreted as the solution of an optimization problem \cite{abgrall2022reinterpretation} or as an additional viscosity/anti-viscosity term. 
Inspired by \cite{abgrall2018general}, we introduce an entropy correction term with artificial 
diffusion into the corrector of the ADER formulation \eqref{eq:ADER-DG} using a generic element $\psi$ from our underlying approximation space.  It yields
\begin{equation}\label{eq:ADERupdateDiffusion}
	\begin{aligned}
	& \int_{\Omega_i} \psi  (\x)
	\left( \u_h^{n+1}(\x) - \u_h^{n}(\x) \, \right) \, \diff \x 
	+ \int_{t^n}^{t^{n+1}} \!\! \int_{\partial \Omega_i} \!\! \psi(\x) \mathcal{F}_{\mathbf{n}}\left(\q_h^-(\x,t), \q_h^+(\x,t) \right) \, \diff S \, \diff t \ - \\
	& \int_{t^n}^{t^{n+1}} \!\! \int_{\Omega_i } \!\!\! \nabla \psi(\x)\cdot \F(\q_h(\x,t))  \diff \x \,\diff t 
	+   \int_{t^n}^{t^{n+1}}\!\! \alpha_{\Omega_i}\int_{\Omega_i}\nabla \psi(\x) \, A_0\, \nabla \v_h(\q_h(\x,t))  \, \diff \x \,\diff t 
	\, =\,  \mathbf{0},
	\end{aligned}
\end{equation}
where $\v_h$ is the approximation of the entropy variables $\v\in \R^{m}$ and $A_0\in \R^{m\times m}$ is a positive definite matrix\footnote{To obtain dimensionally correct terms, the inverse of the Hessian of the entropy $\eta_{\U\U}$ evaluated in an average value of the cell will be used.}.
Using some quadrature formula for the time integration, from \eqref{eq:ADERupdateDiffusion} we obtain 
\begin{equation}
	\begin{aligned}
		& \int_{\Omega_i} \psi  (\x)
		\left( \u_h^{n+1}(\x) - \u_h^{n}(\x) \, \right) \, d\x 
		+ \Delta t \sum_{s=0}^S\beta_s \int_{\partial \Omega_i} \!\! \psi(\x) \mathcal{F}_{\mathbf{n}}\left(\q_h^{s,-}(\x), \q_h^{s,+}(\x) \right)  \, \diff S  - \\
		& \Delta t \sum_{s=0}^S \beta_s  \!\!\int_{\Omega_i} \nabla \psi(\x)\cdot \F(\q^s_h(\x)) \,\diff \x
		+ \Delta t \sum_{s=0}^S \beta_s \,\alpha^s_{\Omega_i}  \int_{\Omega_i} \nabla \psi(\x) A_0 \nabla \v_h(\q^s_h(\x)) \diff \x
		\, =\,  \mathbf{0},
	\end{aligned}
\end{equation}
where $\beta_s$ are the time quadrature weights.
It is left to define all $\alpha_{\Omega_i}^s$. We choose them in order to have an entropy dissipative (conservative) semi-discretization update.
This means that at each 
subtimestep $t^{n,s}$, substituting $\psi = \v_h(\q^s_h(x))$ and summing over the variables, we should have
\begin{align}
	&\int_{\partial \Omega_i} \!\!  \inner{\v_h(\q^s_h(\x)), \mathcal{F}_{\mathbf{n}}\left(\q_h^{s,-}(\x), \q_h^{s,+}(\x) \right) } \, \diff S  - 
	\!\!\int_{\Omega_i} \nabla  \v_h(\q^s_h(\x)) : \F(\q^s_h(\x)) \,\diff \x +\\
	%+ \int_{t^n}^{t^{n+1}} \!\! \int_{\Omega_i^{\circ} } \phi_k \mbf{{B}}(\q_h) \cdot \nabla \q_h \,d\x\,dt 
	&\alpha^s_{\Omega_i} \int_{\Omega_i}  \nabla  \v_h(\q^s_h(\x))^T A_0 \nabla \v_h(\q^s_h(\x)) \diff \x
	\, \geq \,  \int_{\partial \Omega_i} \mathcal{G} (\v_h(\q^{s,-}(\x)),\v_h(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S,
\end{align}
where $\mathcal{G}$ is a consistent  numerical entropy flux.
In order to achieve this, we split the numerical flux into a central part and a diffusive one as 
\begin{equation}
	\mathcal{F}(\q^+,\q^-)\cdot \mathbf{n} = \mathcal{F}^c_{\mathbf{n}}(\q^+,\q^-)+\mathcal{F}^d(\q^+,\q^-).
\end{equation}
As an example with a {local Lax-Friedrich (Rusanov)} entropy type flux, we would have 
\begin{equation}\label{eq:numericalFluxParts}
		\mathcal{F}^c_{\mathbf{n}}(\q^+,\q^-):= \frac{\mathbf{F}(\q^+)+\mathbf{F}(\q^-)}{2} \cdot \mathbf{n}, \ \text{ and }\
	 \mathcal{F}^d(\q^+,\q^-):= -\mathbf{a}_{LF}(\q^+,\q^-) \frac{\q^+-\q^-}{2}
\end{equation}
with $\mathbf{a}_{LF}$ the spectral radius of the flux Jacobian. \\
For simplicity, we introduce the following definitions of the central spatial contribution, the diffusion flux term and the entropy fix  
\begin{align*}
	&\mathtt{F}_{i}^s:= \int_{\partial \Omega_i} \!\! \left\langle \v_h(\q^s_{h,i}(\x)) , \mathcal{F}^c_{\mathbf{n}}\left(\q_h^{s,-}(\x), \q_h^{s,+}(\x) \right) \right\rangle \, dS  \ - \!\! \int_{\Omega_i^{\circ} } \!\!\! \nabla \v_h(\q_h^s(\x)) : \F(\q_h^s(\x)) \,d\x,\\
	&\mathtt{D}_{i}^s:= \int_{\partial \Omega_i} \!\left \langle\v_h(\q^s_{h,i}(\x)),  \mathcal{F}^d\left(\q_h^{s,-}(\x), \q_h^{s,+}(\x) \right) \right\rangle \, dS , \\
	& \mathtt{E}_{i}^s:= \int_{\Omega_i} \nabla \v_h(\q^s_h(\x))^T\, A_0\, \nabla \v_h(\q_h^s(\x)) \,d\x  \geq 0.
\end{align*}
With these definitions, we can finally determine $\alpha_{\Omega_i}^s$ in such a way to ensure entropy conservation or entropy dissipation.
We start focusing on the entropy dissipative case, therefore
a simple choice would be to determine $\alpha_{\Omega_i}^s$  such that the entropy contribution of the central part vanishes, i.e.,
\begin{equation}
	\int_{\partial \Omega_i}\mathcal{G}(\v_h(\q^{s,-}(\x)),\v_h(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S= \mathtt{F}_i^s + \alpha_{\Omega_i}^s \mathtt{E}_i^s, \qquad s=1,\dots, S.
\end{equation}
This leads to the definition of 
\begin{equation}\label{eq:alpha_i-s}
	\alpha_{\Omega_i}^s =\frac{\int_{\partial \Omega_i}\mathcal{G}(\v(\q^{s,-}(\x)),\v(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S- \mathtt{F}_i^s}{\mathtt{E}_i^s}.
\end{equation}
\begin{comment}
\MR{{\bf Nota bene:} This definition ensures the respect of a semi-discrete  (time-continuous) \emph{local}  conservation law
which can be written  within the accuracy of the  quadrature formula in time as 
\begin{equation*}
\begin{aligned}
	\Delta t \sum_{s=0}^S \beta_s   \int_{\Omega_i}& \v_h^s(\x)^T\partial_t \u_h(\x, t^s)  \, \diff \x + 
\Delta t \int_{\partial \Omega_i}  \sum_{s=0}^S \beta_s    \mathcal{G}(\v(\q^{s,-}(\x)),\v(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S
		+  \sum_{s=0}^S \beta_s \mathtt{D}_i^s  =0
	 \end{aligned}
\end{equation*}
To make it fully discrete we can further correct, and in particular set
\begin{equation}\label{eq:alpha_i-s2}
	\alpha_{\Omega_i}^s =\frac{\int_{\partial \Omega_i}\mathcal{G}(\v(\q^{s,-}(\x)),\v(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S- \mathtt{F}_i^s}{\mathtt{E}_i^s} +
\frac{\int_{ \Omega_i}(\eta^{n+1}_h-\eta_h^n)^s /\Delta t-\int_{\Omega_i} \v_h^s(\x)^T\partial_t \u_h(\x, t^s)  \, \diff \x }{\mathtt{E}_i^s} 	.
\end{equation}
{\bf To be written more carefully concerning the time levels for $\eta$,  and checked for possible local conservation.}}
\end{comment}
Since the diffusive part $\mathtt{D}_{i}^s$ decreases always the entropy, we obtain the following estimation
\begin{equation*}
\begin{aligned}
	\int_{t^n}^{t^{n+1}} \int_\Omega& \v_h(\x,t)^T\partial_t \u_h(\x,t)  \, \diff \x  \approx - \Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega} \left(\mathtt{F}_i^s + \alpha_{\Omega_i}^s \mathtt{E}_i^s + \mathtt{D}^s_{i}\right) \\
	 &=- \Delta t \sum_{s=0}^S \beta_s \left[  \sum_{\Omega_i \in \Omega}\int_{\partial \Omega_i}     \mathcal{G}(\v(\q^{s,-}(\x)),\v(\q^{s,+}(\x))) \cdot \mathbf{n}\, \diff S + \sum_{i\in \Omega} \mathtt{D}_i^s \right] \leq - \Delta t \sum_{s=0}^S \beta_s \int_{\partial \Omega}     \G(\v(\q^s(\x))) \cdot \mathbf{n}\, \diff S.
	\end{aligned}
\end{equation*}
With this definition, we correct the contribution from the centered term of the numerical flux. In particular, we are able to split the update into an entropy conservative part ($\mathtt{F}_i^s+\alpha_{\Omega_i}^s \mathtt{E}_i^s$) and an entropy dissipative part ($\mathtt{D}_i^s$). 
This splitting will be crucial when introducing the relaxation technique, as it allows to choose which part we need to balance also in time. 
\begin{comment}

If we removed the $\mathcal{F}^d$ term in the numerical flux,
this correction would allow us also to obtain an entropy conservative spatial discretization,  independently on  the exactness of the numerical quadrature, and without
resorting to any split form to enforce some summation by parts property. The inclusion of the dissipative term of the flux
allows to verify the inequality at the continuous (in time) level.\\
If entropy conservation is the property sought, we can also proceed differently and keep the $\mathcal{F}^d$ term in the numerical flux as well as in
 the definition of $\alpha_{\Omega_i}^s$ leading to the following %to have an entropy conservative spatial discretization. The 
 definition of $\alpha_{\Omega_i}^s$:% become then
\begin{equation}
	\alpha_{\Omega_i}^s =\frac{\int_{\partial \Omega_i}\mathcal{G}(\v(\q^{s,-}(\x)),\v(\q^{s,+}(\x))) \cdot \mathbf{n}\, d S- \mathtt{F}_i^s-\mathtt{D}_i^s}{\mathtt{E}_i^s}.
\end{equation}
In this case, the 
 integral of entropy variation is 
\begin{equation*}
	\int_{t^n}^{t^{n+1}} \int_\Omega \v_h(\x,t)^T\partial_t \u_h(\x,t)  \, \diff \x   \approx    - \Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega} \left(\mathtt{F}_i^s + \alpha_{\Omega_i}^s \mathtt{E}_i^s + \mathtt{D}^s_{i} \right) =  - \Delta t \sum_{s=0}^S \beta_s \int_{\partial \Omega}     \G(\v(\q^s(\x))) \cdot \mathbf{n}\, \diff S.
\end{equation*}
In this case, we balance the entropy conservation in a semi-discrete way. 
\end{comment}
\begin{remark}[Division by zero]
	The division performed in \eqref{eq:alpha_i-s} is numerically dangerous as in flat areas $\normalfont \texttt{E}_i^s$ might be 0. In order not to risk to encounter NaN, we perform that division only if $\normalfont \texttt{E}_i^s \geq \varepsilon^s$, otherwise we set $\alpha_{\Omega_i}^s =0$. This tolerance $\varepsilon^s$ is chosen in the following way
	\begin{equation}
		\varepsilon^s : = \bar{h}^{\,N} \max_{i\in \Omega} \normalfont \texttt{E}_{i}^s,
	\end{equation}
where $N$ is the polynomial degree and $\bar{h}$ is the average mesh size. This guarantees not to introduce extra terms where the solution is constant or almost constant. 
\end{remark}

\begin{remark}[Correction for first order finite volume schemes]
	The special case of $N=0$, i.e., the finite volume method, does not fit in our framework as the terms $\mathtt{E}$ are all zero.
	In this case, we can resort to the classical characterization by Tadmor \cite{tadmor1987numerical,tadmor_2003}.  
	On unstructured grids we introduce  the jumps  $[\! [ (\cdot) ]\!] = (\cdot)^+ -(\cdot)^- $ on a given mesh face with 
	 normal $\n_f$. The generalization of the classical Tadmor condition \cite{ray2016entropy, tadmor_2003}
	 \begin{equation}\label{eq:Tadmor_FV}
	 [\![ \v_h]\!]^T\mathcal{F}^{co}_{\mathbf{n}_f}  = [\![ \pmb{\psi}(u_h)]\!] \cdot \n_f
	 \end{equation}
             defines an entropy conservative flux $\mathcal{F}^{co}$ consistent with the numerical entropy flux
              \begin{equation}\label{eq:Tadmor_FV_EC}
	 \mathcal{G}_{\n_f}  :=   \overline{\v}_h^T\mathcal{F}^{co}_{\mathbf{n}_f}  - \overline{\pmb{\psi}}(u_h)\cdot \n_f,
	 \end{equation}
       having denoted by $\overline{\cdot}$ the arithmetic average, and by $\pmb{\psi}$ the  entropy potential defined by
              \begin{equation}\label{eq:E-potential}
              \G = \v^T\F -\pmb{\psi}.
	 \end{equation}              
	 A given numerical flux $\mathcal{F}_{\n_f}$ may not verify \eqref{eq:Tadmor_FV}. However, we can use the  face jumps  as a correction term and define
	\begin{equation}\label{eq:FV-correction}
		\mathcal{F}^{co}_{\mathbf{n}_f}=  \mathcal{F}_{\mathbf{n}_f} -  \alpha_f  A_0 (\v^+ - \v^-) =\mathcal{F}_{\mathbf{n}_f} -  \alpha_f  A_0 [\![\v]\!].
	\end{equation}
	By imposing the entropy conservation condition \eqref{eq:Tadmor_FV}, we compute a limiting value 
%	where the face $f_{ij}$ belongs to the cell $i$ and $j$.
%	Multiplying by the entropy variables, one obtains an entropy balance that leads to the definition of 
%
%	\begin{equation}\label{eq:correction-pnpm-i}
%		\alpha_f =  \dfrac{ \int_{f}  \left(  [\![\v_h^T ]\!]   \mathcal{F}(\u_h^{-}, \u_h^{+})   - [\![\v_h^T\F(\u_h ) ]\!] \right)\cdot \mathbf{n}_f  }{\big\|  [\![\v_h]\!] \big\|^2_{L^2(f, A_0)}   }
%	\end{equation}
%	while global semi-discrete entropy stability is obtained for $\alpha_f > \alpha_0$.
%	In the DG$0$ case  the expressions simplify quite a bit. For a face between elements $i$ and $j$ we get 
	\begin{equation}\label{eq:correction-pnpm-j}
		\alpha_0  := \dfrac{ - [\![ \pmb{\psi}]\!] \cdot\n_f  + [\![\v]\!]^T \mathcal{F}_{\mathbf{n}_f}   }{[\![\v]\!]^TA_0[\![\v]\!]} =
		\dfrac{ [\![ \G]\!] \cdot \n_f - [\![\v_h^T\F ]\!] \cdot\n_f  + [\![\v]\!] ^T\mathcal{F}_{\mathbf{n}_f}   }{[\![\v]\!]^TA_0[\![\v]\!]} .
	\end{equation}
		Entropy conservation is ensured  for $\alpha_f=\alpha_0$,  	while  semi-discrete entropy stability is obtained for $\alpha_f > \alpha_0$.
	Note that this  comparison result is relatively classical, see \cite{tadmor_2003}.
	In this work, we will focus on high order methods, and we will not discuss further this case. The authors are anyway considering this formulation to obtain an \textit{a posteriori} subcell finite volume limiter, in order to deal with solutions with strong shocks. This will be object of future studies, as the coupling of the two techniques is delicate and must be handled carefully. 
\end{remark}  

%\red{Should we write that this could be the starting point for an a posteriori subcell FV limiter, which however is not the bobject of this work because all the coupling is delicate?}


\subsection{Relaxation applied to ADER-DG}
Would the time integration be exact (vis in the time continuous case), the correction introduced in the previous section would allow to satisfy
\emph{exactly} entropy conservation/stability within each element. But, unfortunately, in general this is not the case and moreover 
the fully discrete nature of the ADER approach requires to handle the temporal discretization simultaneously with the spatial one.
To achieve exact entropy conservation thus we adapt 
%
%Finally, we have to balance the entropy production/distruction that the time-integration introduces in our ADER-DG scheme.
% Therefore,  %we apply
 the relaxation approach proposed in \cite{ketcheson2019relaxationRK}, and applied in different contexts %in 
 \cite{abgrall2021relaxation, kang2021entropy, ranocha2020relaxationRKEuler, ranocha2020relaxationMultistep}.
The key idea of the relaxation ansatz is to project the final numerical approximation $ \u^{n+1}_h$ back to the manifold where the entropy is constant (or dissipative), as in  the underlying continuous setting. 
This is obtained multiplying the time-step $\Delta t$ with a scalar quantity $\gamma^n$ and using this new time-step for the update. 
We describe now how $\gamma^n$ can be chosen in order to preserve (or dissipate) the total entropy \eqref{eq:total_U}.
We set 
\begin{equation}
	\Delta \u_h := \u^{n+1}_h -\u^{n}_h, 
\end{equation} 
where $\u^{n+1}_h$ is obtained solving \eqref{eq:ADERupdateDiffusion}. Now, we have to find 
$\gamma^n$ and $\u^{n+1}_{h,{\gamma^n}} := \u_h^n + \gamma^n \Delta \u_h $ such that the total entropy is controlled. We start by estimating the total entropy \eqref{eq:total_U} as
\begin{align}
	\mathcal{E}(\urp) &= \int_{\Omega} \eta(\urp) d\x \approx \int_{\Omega} \eta(\un) d\x+ \gamma^n \langle \eta_u(\un) ,\ud \rangle \diff \x \\
	&\approx \mathcal{E}(\un) - \gamma^n \Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega} \left(\mathtt{F}_i^s + \alpha_{\Omega_i}^s \mathtt{E}_i^s + \mathtt{D}^s_{i} \right) \\
	&\leq \mathcal{E}(\un) -\gamma^n\Delta t \sum_{s=0}^S \beta_s \int_{\partial \Omega } G(\v^s) \cdot \mathbf{n} \diff S \approx \mathcal{E}(\un) -\int_{t^n}^{t^{n+1}_{\gamma^n}}  \int_{\partial \Omega} G(\v^s) \cdot \mathbf{n} \diff S.
\end{align}
This leads us to the following (non-)linear equation: %, we want to maintain
\begin{equation}\label{eq:ADERgammaEquation}
	\mathcal{E}(\urp) = \int_{\Omega}  \eta(\un +\gamma^n \ud )d\x \stackrel{!}{=} \int_\Omega \eta(\un)\diff \x - \gamma^n\Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega}  \left(  \mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s +\mathtt{D}_{i}^s \right).
\end{equation}
This is equivalent to finding the zero of %i.e., we want to find the zero of
\begin{equation}\label{eq:relaxation_residual}
	R(\gamma^n):= \int_{\Omega}  \eta(\un +\gamma^n \ud )d\x -\int_\Omega \eta(\un)\diff \x + \gamma^n\Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega}  \left(  \mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s +\mathtt{D}_{i}^s \right).
\end{equation}
In case we want to exactly preserve the entropy in time, we can remove the $\mathtt{D}_i^s$ terms from equation \eqref{eq:ADERgammaEquation}.
From \eqref{eq:ADERgammaEquation}, we can finally calculate $\gamma^n$ at every time-step and we update the new value of the approximated solution and the new time-step via 
\begin{equation}\label{eq:update_relax}
\begin{cases}
	\tilde{\u}^{n+1}_{h,\gamma^n} := \un + {\gamma^n} \Delta \un,\\
	\tilde{t}^{n+1}_{\gamma^n} := t^n + {\gamma^n} \Delta t.
\end{cases}	
\end{equation}


\begin{remark}[Division by zero (Relaxation)] As discussed in Remark 4.1, when $\mathtt{E}_i^s< \varepsilon$ we set  $\alpha_{\Omega_i}=0$.
To ensure control of the entropy production up to machine accuracy this particular case needs to be treated also in the relaxation procedure.
In our approach, if $\mathtt{E}_i^s< \varepsilon$ we replace  $\mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s $
by $\int_{\partial \Omega_i} G(\v^s)\cdot \mathbf{n} \diff S$ in  \eqref{eq:ADERgammaEquation}. This guarantees that we still have 
%Then, if \eqref{eq:ADERgammaEquation} is verified, we will have that 
\begin{equation}
	\mathcal{E}(\urp) = \mathcal{E}(\u^n_h) - \sum_{s=0}^S \beta^s \left[ \int_{\partial \Omega} G(\v^s) \cdot\mathbf{n} \,\diff S + \sum_{\Omega_i \in \Omega} \mathtt{D}_i^s \right],
\end{equation}
which is otherwise guaranteed by the definition of  $\alpha_{\Omega_i}$.
\end{remark}
 
%
%Note that if $\alpha_{\Omega_i}$ was set to 0 because $\mathtt{E}_i^s< \varepsilon$, then, in \eqref{eq:ADERgammaEquation} we put $\int_{\partial \Omega_i} G(\v^s)\cdot \mathbf{n} \diff S$ instead of $\mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s $.
%Then, if \eqref{eq:ADERgammaEquation} is verified, we will have that 
%\begin{equation}
%	N(\urp) = N(\u^n_h) - \sum_{s=0}^S \beta^s \left[ \int_{\partial \Omega} G(\v^s) \cdot\mathbf{n} \,\diff S + \sum_{\Omega_i \in \Omega} \mathtt{D}_i^s \right].
%\end{equation}


It should be pointed out that in case of quadratic entropies \eqref{eq:ADERgammaEquation}  is explicitly solvable as demonstrated in Example \ref{ex.quadratic} below, while for more nonlinear entropies a nonlinear solver for the scalar equation \eqref{eq:ADERgammaEquation} must be used. In our numerical simulations in Section \ref{sec.test}, we use a simple Newton method to solve \eqref{eq:ADERgammaEquation}. 
\begin{remark}[Newton method for \eqref{eq:relaxation_residual}]
	When we want to find the (non trivial) zero of \eqref{eq:relaxation_residual}, the Newton method or variants can help in finding the solution. For Newton method also the derivative of $R$ is required, but it is easily computable as
	\begin{equation}
		\frac{dR(\gamma^n)}{d\gamma^n} = \int_{\Omega}  \left\langle \v(\un +\gamma^n \ud ),\ud \right\rangle d\x  +\Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega}  \left(  \mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s +\mathtt{D}_{i}^s \right).
	\end{equation}
\end{remark}In that case, to compute the Jacobian, the entropy variable definition is, again, necessary.
Finally, we have to stress out that due to the results of \cite{ranocha2020relaxationMultistep}, we can ensure that
if the underlying time method is of order $p\geq2$,
\begin{itemize}
\item there exists always a unique $\gamma>0$ that solves \eqref{eq:ADERgammaEquation}. This $\gamma$ satisfies $\gamma=1+ \mathcal{O}(\Delta t^{p-1})$ under a reasonable small time-step $\Delta t$, and 
\item the relaxation solution $\tilde{\u}^{n+1}_{h,\gamma^n} $ is also of order $p$.  
\end{itemize}

Using now both, the entropy correction terms and the relaxation approach, we obtain an entropy preserving ADER-DG method for which we will verify the properties next in the numerical experiments section, but before we finish this part with the following already mentioned example. 


\begin{example}[Quadratic entropy]\label{ex.quadratic}
	In case of a quadratic entropy for scalar equations 
	$$
	\eta(u) :=\frac{ \langle u, u \rangle }{2},
	$$
	we can exploit the expression $\mathcal{E}(\urp)$ as
	\begin{align}
		\mathcal{E}(\urp)& = \int_{\Omega} \eta(\un +\gamma^n \ud ) d\x = \frac{1}{2} \int_{\Omega} \langle  \un +\gamma^n \ud ,  \un +\gamma^n \ud \rangle  \\
		&= \frac{1}{2}\int_{\Omega} \langle  \un ,  \un \rangle  + 2 \gamma^n \langle  \ud ,  \un \rangle  + (\gamma^n)^2 \langle \ud ,\ud \rangle d \x  \\
		&= \mathcal{E}(\un) + \int_{\Omega}  \gamma^n \langle  \ud ,  \un \rangle  + \frac{1}{2}(\gamma^n)^2 \langle \ud ,\ud \rangle d \x,
	\end{align}
   so that \eqref{eq:ADERgammaEquation} reduces to
   \begin{align}
   	\int_{\Omega}  \gamma^n \langle  \ud ,  \un \rangle  + \frac{1}{2} (\gamma^n)^2 \langle \ud ,\ud \rangle \diff \x \stackrel{!}{=} -\gamma^n\Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega}  \left(  \mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s +\mathtt{D}_{i}^s \right).
   \end{align}
	The solution $\gamma^n=0$ is not the one we search, the other one is
	\begin{equation}\label{eq_gamme_energy}
		\gamma^n =-2 \frac{\Delta t \sum_{s=0}^S \beta_s \sum_{i\in \Omega}  \left(  \mathtt{F}_{i}^s+\alpha_{\Omega_i}^s\mathtt{E}_{i}^s +\mathtt{D}_{i}^s \right)+\int_{\Omega} \langle  \ud ,  \un \rangle \diff \x }{\int_{\Omega} \langle \ud ,\ud \rangle d \x},
	\end{equation}
	which is close to one. 
\end{example}




%\subsection{On the practical implementation of the  correction and relaxation terms}





==> Hyperbolic.tex <==

Various natural phenomena and engineering problems can be described by the following system of hyperbolic conservation laws
\begin{equation}
\label{eq.generalform}
\partial_t\u+ \operatorname{div} \F (\u)= 0,
\end{equation}
where $\u: \Omega \times \R^+ \to \Psi \subset \R^m$ denotes the conserved variable depending on the space coordinate $\x \in \Omega \subset \R^D $ and time coordinate $t \in R^+$, $\F:\Psi\to \R^{D\, \times\, m}$ is the flux function and $\operatorname{div}$ is the divergence operator. As usual, system  \eqref{eq.generalform} is  equipped with appropriate boundary and initial conditions.  
In the scalar case we 
 will use the symbol $u$ for the conservative variable. 
The paper focuses on the two-space dimensional problems \eqref{eq.generalform}, i.e. $\Omega \subset \R^2$. 
However note that all the ideas presented  readily apply to the general case.  In the simulation section, we will show test on scalar linear advection equation, shallow water equations and gas dynamic Euler's equations. All the details on the equations are described in that section.\\
%We will consider examples for hyperbolic conservation laws ranging from the scalar linear advection equation 
%\begin{equation}\label{eq:advection}
%	\partial_t U +  \partial_x (a_1 U)+ \partial_y (a_2 U)  = 0,
%\end{equation}
%where $a_1$ and $a_2$ are constants,  to the Euler equations of gas dynamics 
%\begin{equation}\label{eq_Euler_conservation}
% \begin{aligned}
%   \partial_t \rho +\div \bm&=0,\\
%   \partial_t \bm +\div \left( \frac{\bm\otimes \bm}{\rho} \right) +(\gamma-1) \nabla_x \left(
%   E-\frac{1}{2} \frac{|\bm|^2}{\rho}\right)&=0,   \Longleftrightarrow \qquad \partial_t \U+\div \F=0.\\
%   \partial_t E +\div \left [\left( E +(\gamma-1)\left(
%   E-\frac{1}{2} \frac{|\bm|^2}{\rho}\right) \right) \frac{\bm}{\rho} \right]&=0.
% \end{aligned}
%\end{equation}
%
%\red{We said that maybe we could let the details on Euler equations for the numerical results section and stay more general here}
%
%Here, $\rho$ denotes the density, $\bm=\rho \u \in \R^d$ the momentum, 
%$E=\frac{1}{2} \rho |\u|^2 +\rho e$ the total energy,  $e$ the internal energy, $\u:=(u_1, u_2)^T$ the velocity field
%and $\gamma>1$ the adiabatic constant. $\U=(\rho, \bm, E)^T$ is the conservative variable
%and the flux function is given by $\F_d=(\rho u_d, u_d \bm +p \mathbf{I}_d, u_d(E+p))^T$ with $d=1,2$,
%and pressure 
%$p=(\gamma-1)\rho e$  as  the equation of state for an ideal gas and $\mathbf{I}_d$ the $d$-th column of the $2\times 2$ identity.\\
Due to the non-uniqueness of weak solutions of \eqref{eq.generalform}, the concept of entropy as an additional admissible criterion is necessary.
Following the classical paper \cite{harten1983symmetric}, 
 $\eta \colon  \Psi \to \R$ is a convex entropy function with related entropy flux $\G$ and entropy variable $\v= \partial_\u \eta$ verifying $\scp{\v}{\partial_\u  \F_d }=\partial_\u \mathbf{G}_d$.
 Smooth solutions of \eqref{eq.generalform}  fulfill additionally  the entropy conservation law
\begin{equation}
\label{eq.generalform_entropy_conservation}
\partial_t \eta + \div  \G = 0,
\end{equation}
while admissible weak solutions are  characterized by the entropy inequality 
\begin{equation}
\label{eq.generalform_entropy_inequality}
\partial_t \eta + \div \G \leq 0.
\end{equation}
If $\eta$ is  strictly convex, the mapping between the entropy variables $\v =\partial_\u \eta$ and the conservative variables $\u$ is one-to-one. We can either work directly with $\v$ or  $\u$ when solving \eqref{eq.generalform}. Moreover, it holds that the Hessian $\partial_{\u\u}\eta$ (or Jacobian $\partial_\u \v$) is a symmetric positive definite (SPD) matrix and we denote
its inverse by $A_0:= \partial_{\v}\u.$
Finally, our numerical approximations will be constructed in a way to solve 
\eqref{eq.generalform} and fulfill the entropy conditions \eqref{eq.generalform_entropy_conservation} or \eqref{eq.generalform_entropy_inequality} in a global manner. Introducing the total entropy $\mathcal{E}$ defined by the integral
\begin{equation}
\label{eq:total_U}
\mathcal{E}(\u)=\int\limits_{\Omega}\eta(\u)\diff \x ,
 \end{equation}
 total entropy conservation stems immediately from \eqref{eq.generalform_entropy_conservation} and reads
\begin{equation}
\label{eq.global_entropy_conservation}
%\partial_t N(\u) + \int\limits_{\partial\Omega}  \G\cdot\hat{\mathbf{n}} \;\diff S = 0,
\partial_t \mathcal{E}(\u) + \int\limits_{\partial\Omega}  \G\cdot\hat{\mathbf{n}} \;\diff S = 0.
\end{equation}
Our objective is to provide a strategy allowing to design ADER-DG schemes capable to mimic the last identity  within machine precision.

 


==> Introduction.tex <==


In last years, the development of arbitrary high-order entropy preserving discretizations
has attracted a lot of attention in community developing numerical methods for % been a major task inside the
hyperbolic PDEs. % research community. 
Following the seminal work by Tadmor \cite{tadmor1987numerical,tadmor_2003}, several ideas have surfaced providing general strategies to have control
on the discrete production of entropy. Many works were focused on finding an entropy stable semidiscretization (in space), isolating the entropy conservative flux. These techniques have been applied to many applications, \textit{inter alia} for shallow water equations \cite{gassner2016well,wintermeyer2017entropy,parisot2019entropy}, for Euler's equation \cite{puppo2011numerical,gassner2016split,chandrashekar2013kinetic,ray2016entropy, chandrashekar2013entropy, crean2018entropy}, Navier Stokes problems \cite{gassner2018br1,yamaleev, fernandez2020entropy, manzanero2020entropy,manzanero2020entropy2}, magneto hydro-dynamics problems \cite{chandrashekar2016entropy}, multiphase or multicomponent problems \cite{coquel2021entropy,renac2021entropy,marmignon2022energy} and generally for hyperbolic problems \cite{abgrall2018general, abgrall2020analysis, kuzmin2021entropy, kuzmin2020algebraic, chen2017entropy, carpenter2014entropy, fisher2013high, fisher2013discretely, kopriva2022theoretical, hillebrand2022comparison, renac2019entropy}, also in the Lagrangian framework \cite{carre2009cell,duan2021entropy,chan2021positivity}.
More recently also fully discrete entropy stable or entropy conservative schemes have been introduced, e.g. \cite{ketcheson2019relaxationRK, ranocha2020relaxationRKEuler, abgrall2021relaxation, abgrall2022reinterpretation, friedrich2019entropy, kuzmin2022limiter}. These techniques exploit quite different underlying mechanisms, e.g.  artificial viscosity, limiting techniques, the summation-by-parts (SBP) framework, entropy correction terms, relaxation ansatzes or combination of those. 
Even if the entropy dissipative methods  differ significantly in their underlying ideas, they have demonstrated excellent numerical properties in numerical simulations. \\
The ADER approach has proved to be an accurate numerical scheme in numerous engineering applications. It has also been shown to be
an appropriate setting to design discretizations 
able to preserve different physical properties. First proposed in \cite{toro2002ader, toro2001towards} as an high-order extension of the classical Godunov scheme, the method has been dramatically extended and re-interpreted in different ways, among which we recall
 \cite{Dumbser20088209, PCSPH, euromech03, boscheri2014high, ALEDG, boscheri2022cell, ADERGRMHD, dumbser2020glm, dematte2020ader, gaburro2021posteriori, chiocchetti2021high}. However, up to this point no provable high-order entropy conservative/dissipative ADER method can be found in the literature. 
Entropy conservation/stability   is  however essential to
 ensure that our numerical approximations converge to the physical relevant weak entropy solution.  In the following work, we will consider this fact and develop for the first time an entropy preserving ADER-DG method. Therefore, we adapt two general techniques to the ADER-DG framework. 
 Inspired by \cite{abgrall2018general, abgrall2022reinterpretation}, we handle the space-discretization of our ADER-DG method  via entropy correction terms whereas the entropy production in time is balanced through the relaxation approach proposed in \cite{ketcheson2019relaxationRK,ranocha2020relaxationMultistep,ranocha2020relaxationRKEuler}.\\
 The %rest of the
  paper is organized as follows. In Section~\ref{sec.hyperbolic}, we briefly 
describe hyperbolic conservation laws and the concept of entropy. Then, in Section~\ref{sec.DG}, the ADER-DG method is introduced in its nowadays used explicit space-time Finite Element (FE) interpretation. In Section~\ref{sec.relaxation_DG}, we describe the applied entropy correction techniques and the relaxation approach used in our ADER-DG framework resulting in a provably entropy preserving method. Next, in Section~\ref{sec.test} we verify our theoretical results via various numerical simulations. A conclusion in Section~\ref{sec.concl} finishes this paper.  
